Genie: A Generator of Natural Language Semantic Parsers for Virtual Assistant Commands

To understand diverse natural language commands, virtual assistants today are trained with numerous labor-intensive, manually annotated sentences. This paper presents a methodology and the Genie toolkit that can handle new compound commands with significantly less manual effort. We advocate formalizing the capability of virtual assistants with a Virtual Assistant Programming Language (VAPL) and using a neural semantic parser to translate natural language into VAPL code. Genie needs only a small realistic set of input sentences for validating the neural model. Developers write templates to synthesize data; Genie uses crowdsourced paraphrases and data augmentation, along with the synthesized data, to train a semantic parser. We also propose design principles that make VAPL languages amenable to natural language translation. We apply these principles to revise ThingTalk, the language used by the Almond virtual assistant. We use Genie to build the first semantic parser that can support compound virtual assistants commands with unquoted free-form parameters. Genie achieves a 62% accuracy on realistic user inputs. We demonstrate Genie's generality by showing a 19% and 31% improvement over the previous state of the art on a music skill, aggregate functions, and access control.

==> conclusion.tex <==
%!TEX root = ./paper.tex

\section{Conclusion}
\label{sec:conclusion}
Virtual assistants that support compound commands can greatly simplify and enhance our lives,
but no usable semantic parser has previously been developed due to the complexity of the commands.
In this paper, we introduce Genie, a toolkit to help developers generate a semantic parser with high accuracy
for a given virtual assistant formal language.

We introduce the concept of natural language templates to bridge the gap between natural language and formal language.
By supplying primitive and construct templates in an iterative fashion, developers can use Genie
to create a large high-quality dataset consisting of synthesized sentences and paraphrased sentences for training.

We also propose design principles for Virtual Assistant Programming Languages that can improve semantic parsing accuracy.  We extend \TT to follow these principles, and show that Genie delivers a semantic parser with 62\% accuracy on realistic inputs, and 63\% on IFTTT data.
We also evaluate Genie on a sophisticated music skill, an extension of \TT with aggregation support, and 
a new formal language for access control.
The semantic parsers generated by Genie obtain at least 67\% accuracy for all three tasks, and improve the baseline by at least 19\%, which 
shows the power and generality of Genie.


==> exec.tex <==
\section{Applying ThingTalk to a Virtual Assistant}

\subsection{Automatically Generated Conversations}

\subsection{ThingTalk Execution Engine}

\subsection{Distributed ThingTalk}


==> guidelines.tex <==
\section{Lessons and Guidelines}

The development of Genie, and the ThingTalk language, was the result of a multi-year refinement process.
In this section, we highlight some of the insights we have learned.

\paragraph{Avoid variable names}
The first iteration of ThingTalk used unification to connect input and output parameters of methods,
rather than parameter passing. Unification was problematic because the variables were given
arbitrary names, that the synthesizer would have to guess, or the user specify the names explicitly in
the sentence. Our current model, instead, uses the declared parameters as the names to use
in parameter passing, and provides a conflict resolution rule to handle joins where two
functions have the same output parameters.

\paragraph{Collapse similar functions and use parameters}
Natural language is inherently ambiguous; if two sentences are similar in meaning, even if the
semantics are slightly different, there is a chance that different people will interpret them
differently. This can affect the quality of the paraphrases, as that depends on the workers
understanding the meaning of synthetic sentences. Worse, if it is possible that two paraphrases
of nominally distinct commands will end up being the same sentence (or almost the same sentence);
that has disastrous effects on the machine learner, which collapses to majority prediction.

This effect can mitigated if similar commands are distinguished by parameters rather than
methods. Specifically, in that case (1) the neural network is not forced to make an immediate
hard decision, and can defer the decision after choosing the function (and receiving positive
reward for it), (2) if the sentence is fully ambiguous, the neural network can a produce a
partially correct answer 100\% of the time, rather than a fully correct answer 50\% of the time.
This improves training and reduces the negative effect of ambiguous sentences in
the training set.

In a similar vein, an earlier iteration of Thingpedia used different methods for streams
and queries on the same data, while the current design uses the \texttt{monitor} operator to distinguish
the stream and query operations. While this introduces more complexity on the runtime,
it improves the training for the parser. Empirically, we observe that even after this
change, about 3\% of our test data is ambiguous with respect of \texttt{now} vs. \texttt{monitor},
so reducing the effect of ambiguity is critical.

\paragraph{Keyword parameters are better than positional parameters}
As consequence of collapsing similar semantics, methods can have many different combinations
of parameters that are meaningful in natural language, with some parameters potentially optional
as well.

If the programming language uses positional parameters, then the neural network has to predict
``undefined'' or placeholder values in place of omitted or unspecified parameters; in turn,
this requires the network to learn the exact signature of each function, both order and length.
The signature information is not generalizable across functions, hence the neural network would need massive
amounts of data \textit{for each function} to learn it. Conversely, when using keyword
parameters the neural network does not need to learn the length of the signature
at all, and the order of parameters in the prediction is defined globally by the normalization
algorithm; hence, the language model of parameters can generalize across functions.

The downside of keyword parameters is that parameters with similar usage across functions
must use the same name, or else the network will need more function-specific data.
In our documentation, we instruct developers on the naming convention to use, and we provide
examples to follow for common cases; we have not found yet this aspect to be problematic.

\paragraph{Expand the synthetic set}
An earlier design of Thingpedia used the single confirmation sentence for a method to generate
the synthetic set, and relied on paraphrasing to expand the set of understood sentences.
We found that to be insufficient, because most of the time paraphrasers make small changes
to input sentence, adjusting the grammar or changing individual words or constituents, or
make the same predictable high-level change, such as flipping the order of when-phrases.

The combination of code snippets and many synthetic templates expands on the space of
sentences shown to the paraphrases, which in turn increases the variety of the training
set, resulting in overall better quality. We have refined the templates by looking at
the previously constructed paraphrased sets, and combined it with domain-specific knowledge;
our iterative approach should generalize to any domain.


==> impl.tex <==
\section{Practical Considerations}
\label{sec:impl}

Genie is a complex tool, involving many components (a programming language, a dataset generation tool, and a semantic parser) written in different languages and frameworks, with different engineering requirements. In this section, we describe some of the practical considerations that we found to be useful in designing Genie.

\subsection{Design of \TT}
In addition to the high level design principles described in Section~\ref{sec:vapl-principles}, there are some practical aspects that matter when designing a \VAPL.
First of all, to support argument identification, the syntax of the language must support named constants such as ``NUMBER\_0'', ``DATE\_1'', etc., which refer to a specific value that has been identified in the input sentence. Second, when a parameter value cannot be identifier deterministically in the sentence, the syntax of the language must support copying words from the input; to do so, string parameters must be tokenized in a way that is compatible with the tokenization of the input. Concretely, each word in a string parameter is an individual token in the \TT grammar.

\VAPL{} should also be easy to manipulate; to a limited extent, should be possible to apply program transformations without parsing the full language into a parse-tree, and then serializing it again. The ability to transform programs without writing a grammar allows rapid prototyping of language features. In \TT, it also responds to the practical need to use multiple programming languages: Genie is written in a mix of JavaScript, Java and Python, and it would be impractical to write a \TT library in each language. Because different open-source communities (such as IoT and ML) have different language preferences, we expect this interoperability requirement will apply to many \VAPL{}s. \TT provides easy manipulation by prefixing each user-defined identifier with a marker that indicates whether it is a function name, parameter name, or enum value. A script can then identify all functions, all parameter names, or all constants, in a program, without understanding the whole language.

With these restrictions and design choices, the syntax of \NLPL{}s becomes unwieldy to write by hand. For this reason, we expect \NLPL{}s to also introduce a second syntax that is less restrictive, including syntactic sugar and allowing programs in non-canonical form. Conversion from one syntax to the other should be possible automatically.

\subsection{Sentence Generator}

The implementation of the sentence generator responds to three concrete requirements: its performance should scale to a large and growing library, it should generate a dataset small enough that it will not overcrowd the paraphrase set, but it should include some amount of complex sentences to expose the model to in training. In this section, we describe the implementation, and how we achieve this balance.

\paragraph{Generation Algorithm}
The sentence generator algorithm is based on the \textit{Floating Parser} algorithm introduced by Pasupat et al.~\cite{pasupat2015compositional}, and later used by Wang et al.~\cite{overnight} to generate canonical forms for paraphrasing. This algorithm expands the templates in a bottom-up fashion, by incrementally constructing lists (\textit{charts}) of intermediate derivations, starting from the templates that only include terminals in their body (primitive templates, and construct templates for constants), and incrementally proceeding to the root. Each chart is associated with a template and a depth; expanding a template into a chart is performed by recursively enumerating all the charts of its non-terminal constituents of lower depth. The algorithm terminates when all possible derivations have been generated, or when a maximum depth is reached.

\paragraph{Sampling Strategy}
Previous work by Wang et al.~\cite{overnight} only considered a small grammar and knowledge base, and in the domains it considers it is feasible to recursively enumerate \textit{all} possible derivations, up to a certain depth. Because the number of derivations is exponential in the depth of the tree, and grows quickly with the size of Thingpedia, full recursive enumeration is not feasible for \TT. Instead, Genie uses a sampling strategy, whereas only a subset of elements in each chart is preserved. The desired size of each chart is configurable, and decreases exponentially with increasing depth; this allows Genie to generate a sufficient number of programs of low depth, which provides broad coverage, while also generating some programs at high depth, which injects variance in the synthesized set and expands the set of recognized programs. Developers using Genie can control the sampling strategy by splitting or combining construct templates, using intermediate derivations.

\iffalse
While sampling, Genie does not generate the full unsampled set of derivations at each step, because that could potentially be too large to hold in memory\footnote{Even if it could fit in memory, it would generate enough garbage that most of the process time would be spent doing GC, at which point the GC would declare that not enough progress is being made and abort the process.}. Instead, Genie computes an acceptance probability, and retains a generated derivation with that probability. The acceptance probability must take into account the semantic function, which can also decide to prune the generated derivation, due to type or semantic constraints. Genie computes the acceptance probability based on the desired chart size, the worst-case estimated size, and an estimate of the pruning factor that the semantic function will apply; this estimate is computed from the previous run of the semantic function (at lower depth) and refined while generating the current chart.
\fi


==> intro.tex <==
%!TEX root = ./paper.tex
\section{Introduction}
\label{sec:intro}
\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/running_example.pdf}
\caption{An example of translating and executing compound virtual assistant commands.}
\label{fig:running_example}
%\vspace{-1em}
\end{figure}

Personal virtual assistants let users use natural language to manage their collection of accounts across all their internet services and IoT devices.  This paper asks how we can design virtual assistants for extensibility.  What should be the interface between natural language (NL) and the execution engine of the assistants?  How can we easily extend virtual assistants with new devices and new constructs? More importantly, how can we teach virtual assistants to understand more commands in natural language easily?   

Virtual assistants are commonly based on \textit{semantic parsing}, a machine learning algorithm that converts natural language to a semantic representation in a formal language.
The power, complexity and accuracy of semantic parsers depend on the target language of choice.

The Abstract Meaning Representation~\cite{banarescu2013abstract} and the Alexa Meaning Representation Language~\cite{kollar2018alexa, perera2018multi} model natural language phenomena explicitly. %\TODO{Is phenomena the right word}
They use machine learning to match NL to a representation model which closely matches the semantics of the sentences.  Semantically equivalent sentences have different representations, requiring complex and expensive manual annotation
by experts, who must know the details of the formalism and associated ontology.  Similarly, the virtual assistant execution engine must also deal with the complexity of the language.

At the other end of the spectrum, 
the open-source Almond virtual assistant uses the formal ThingTalk programming language as an intermediate language; it uses a semantic parser to translate natural language to ThingTalk, which can directly be executed~\cite{almondwww17}.  
ThingTalk only has one construct which has three clauses: when some event happens, get some data, and perform some action, each of which can be predicated. This construct combines primitives from the extensible runtime skill library, Thingpedia, currently consisting of over 200 APIs to internet services and IoT devices. Despite its lean syntax, ThingTalk is expressive. It is a superset of what can be expressed with If-This-Then-That (IFTTT)~\cite{ifttt}, which has crowdsourced 250,000 unique compound commands. Fig.~\ref{fig:running_example} shows how a natural-language sentence can be translated into a ThingTalk program, using the set of services in Thingpedia.

However, no usable semantic parser has been developed for this language so far.  The Almond parser requires all parameters to be explicitly quoted, e.g., ``search `pizza' on Bing'', which is a nonstarter, especially for voice inputs.  Furthermore, the accuracy reported was 71\% if the commands contain one function, and 51\% for two on a dataset based on manual paraphrasing of synthetically generated sentences~\cite{almondwww17}.

\begin{figure*}[tb]
\includegraphics[width=0.8\linewidth]{figures/overview.pdf}
\caption{Overview of the Genie Semantic Parser Generator}
\label{fig:overview}
\vspace{-0.5em}
\end{figure*}

\subsection{Semantic Parsers for Virtual Assistants}

This paper advocates the same execution-based approach used in ThingTalk.  We coin the term \NLPL ({\em Virtual Assistant Programming Language}) to refer to languages designed as a target for natural language translation by virtual assistants. The \NLPL{} exposes the full capability of the virtual assistant to the deep-learning neural network, instead of introducing an intermediate representation that needs to be interfaced with by both the parser and the execution engine. 

After experimenting with state-of-the-art machine-learning techniques to build a semantic parser for ThingTalk, we discovered several unique challenges to this problem. In the end, we created \TT, an extension to ThingTalk, which is amenable to natural language translation, and developed new methodologies and techniques to address the following challenges:

\paragraph{Canonical program representation.}
Semantic parsing has been used mainly for answering questions. 
Models in that domain can be tested by executing the target program
under a test environment and comparing the output to check whether two programs are equivalent.
This is unsuitable to any domain where programs have side effects, such as IoT commands.
The output of the model has to be the program itself.  \NLPL programs must have a (unique) canonical form so we can check if the answer is correct syntactically.

\paragraph{Designing \NLPL for amenability to NL translation.} To make NL translation feasible, \NLPL and its libraries need to be designed with the principles of keeping the semantics of components orthogonal, matching non-developers’ mental model, and supporting partial correctness in translation.  

\paragraph{Programmed training data synthesis.} Machine learning requires training data, which is not available for new languages.  
To create a semantic parser for question answering over simple domains, Wang et al.~\cite{overnight} use a syntax-driven approach to create a canonical sentence for each formal program, ask crowdsourced workers to paraphrase canonical sentences to make them more natural, then use the paraphrased sentences to train a machine model that can match input sentences against possible canonical sentences.
This approach is inadequate for virtual assistants, which use powerful constructs to connect many diverse domains, each with its own vocabulary.  It is simply not possible to generate just one canonical natural language that can be understood across different domains. Crowdworkers often paraphrase sentences incorrectly or just make minor modifications to original sentences. Our approach is to introduce an {\em NL-template language} that allows developers to direct the generation of synthetic sentences.  Developers are expected to iterate on their templates after observing the results of paraphrased sentences.

\paragraph{Compositional Neural Network.}
It is infeasible to collect paraphrases for all the sentences supported by a \NLPL language. To the best of our knowledge, we are the first to show how to combine paraphrased and synthetic data to train an effective compositional semantic parser. 

\subsection{The Genie Toolkit}
To facilitate rapid development of virtual assistant capabilities, we encapsulate the semantic parser methodology we developed in a toolkit called Genie. 
Given a definition of a \NLPL language and a set of NL-templates, Genie generates a semantic parser that translates natural language to code for the new language. As shown in Figure~\ref{fig:overview}, it creates a synthetic data set, crowdsources paraphrases, and augments the training data with parameter values. It trains a neural network model and outputs the parameters of the trained model, and in other words, the semantic parser. 

\subsection{Contributions}

The results of this paper include the following contributions: 

\begin{enumerate}
\item
We present the design principles for \NLPL{}s that improve the success of semantic parsing.
We have applied those principles to \TT, and created a semantic parser that achieves an 87\% accuracy on paraphrased data.

\item
A novel NL-template language that lets developers direct the synthesis of training data for semantic parsers of \NLPL languages.

\item
The first toolkit, Genie, that can generate semantic parsers for \NLPL languages with the help of crowdsourced workers.
%It is the first semantic parser that accepts natural language to formal language translation rules to improve the quality of synthetic sentence generation.
By adding synthetic data to paraphrased data in training, and expanding parameters, our neural model achieves an improvement in accuracy of 22.3\%.

%%introduces the use of max-margin and span-level copying mechanism, which each accounts for a 3\% improvement in accuracy.  
\item
Demonstration of extensibility by the success of using Genie to generate effective semantic parsers for a Spotify skill, aggregate functions, and access control.
\end{enumerate}

\subsection{Paper Organization}
The organization of the paper is as follows. Section 2 describes the \NLPL principles, using \TT as example.
Section~\ref{sec:dataset} introduces the Genie data acquisition pipeline, and Section~\ref{sec:impl}
describes the implementation of the Genie tool in detail.
We present experimental results on understanding \TT commands in Section~\ref{sec:eval},
and additional languages and case studies in Section~\ref{sec:case-studies}.
We present related work in Section~\ref{sec:related} and conclusion in Section~\ref{sec:conclusion}.

\iffalse

%For example, this can be used for corporate virtual assistants that help professionals with their tasks using corporate-confidential skills. 

\paragraph{Expressiveness}
Natural language can express very complex tasks succinctly. How much of that complexity can be captured
by the formal language? Can users compose tasks, extend them and compute on them by describing the tasks
in words? The challenge is to design a formal language that is both tractable to develop and implement,
but also expressive enough to capture all the tasks that the user's want, while matching the user's mental
model of the task.

We propose to combine small core language with a large library. The library provides primitive tasks,
which should match the user's model. The core language allows to combine and compute on the primitives,
increasing the expressiveness of the language without coding each and every command individually.

\paragraph{Extensibility}
The web is growing, and so is the Internet of Things, with new devices being developed and released
constantly. To sustain this growth, virtual assistants must be extensible: is it possible to support newer
devices without building a new system from scratch, and without compromising the quality of existing skills?
Ideally, the marginal cost of new devices should be lower over time, as knowledge of existing
devices can transfer to the new ones.

We propose to support extensibility in two directions: by adding new devices to the library, and by adding
new syntax to the core language. In this paper, we experiment with both, and we find that we can achieve
good results with small effort.



The Genie system accepts the following inputs: 
\begin{itemize}
\item
A repository of skills: APIs and NL-Code mappings
\item
Formal language grammar, and NL-Code mappings
\end{itemize}

Genie generates 
\begin{itemize}
\item
Given a natural language sentence, it will generate a program. This includes a slot filling dialog where necessary. 
\item
Given a program, it will generate a natural language describing the program. 
\end{itemize}

While \TT supports significantly more useful commands than existing virtual assistants, \TT is but one of many constructs understood by the semantic parser. To facilitate the extension to other constructs, we have developed an open-source toolkit call Genie to embody the methodology we developed originally for \TT.  To support modularity, Genie adopts Almond's model where the domain of supported natural language sentences is represented simple constructs in a \NLPL language with an extensible library. Genie includes built-in support for \TT and Thingpedia. Developers can extend Thingpedia, subset Thingpedia, or create new skill repositories in the same Genie library format.  They can also extend \TT or define new \NLPL languages.  The use of Genie for non-English semantic parsing is outside the scope of this paper. 

As shown in Figure~\ref{fig:overview}, Genie accepts as input the grammar of \NLPL, the types and signatures of the functions in the skill library, the NL2FL snippets and the NL2FL constructs and possibly sets of possible values to be supplied to the typed parameters.  


Today commercial virtual assistants can only handle simple commands.  To be truly useful, a virtual assistant needs to perform complex tasks that may involve multiple primitives.  Almond suggests using a high-level formal language, called ThingTalk, as an intermediate language in virtual assistants: a semantic parser translates natural language into ThingTalk, which is then executed by the ThingTalk runtime.  
While ThingTalk has a simple construct, it has rich semantics due to its extensible runtime skill library, Thingpedia, consisting of over 200 APIs to internet services and IoT devices. ThingTalk is expressive as it is a superset of what can be expressed with IFTTT, which has crowdsourced 250,000 unique compound commands. 
The success of this approach can greatly enhance the capability of virtual assistants. 
Fig.~\ref{fig:running_example} shows how a natural-language sentence can be translated into a ThingTalk program, using the set of services in Thingpedia.

Semantic parsing has not been formally described in Almond.


\subsection{Semantic Parsing for Compositional Virtual Assistant Commands}

%There are several main challenges.  First, the accuracy of the semantic parser depends on the design of the formal language, so the semantic parser and the language need to be co-designed and evolve together.  Second, there is no existing natural language corpus to train a new formal language. 

{\em NL (Natural-Language) Programmable Language Design}
ThingTalk is different from existing formal languages because it is intended to be generated by a semantic parser from natural language sentences; furthermore, such sentences are uttered by a consumer, and not a developer.  We refer to such formal languages as \NLPL, short for NL (Natural Language) Programmable Language.  
When assembly languages became no longer handwritten but generated by compilers, co-designing of machine instruction sets and compilers led to the RISC revolution.  Here, we need to co-design the semantic parser and the \NLPL languages to create an effective system. 

{\em Training Data Generation}
The second challenge is how do we get a high-quality training data set. 
Semantic parsing on compound virtual assistants has been attempted using IFTTT recipe descriptions.  Due to the low quality of inputs, the best accuracy reported was 3\%~\cite{quirk15}.  
Liang et al.~\cite{overnight} propose \textsc{Sempre}, a methodology that lets users create new parsers for SQL queries on new databases. 
The main idea is to synthesize a sample of possible programs in the formal program and programmatically generate corresponding natural language utterances. These utterances are often clunky; crowdsourced workers are used to paraphrase a subset of these sentences to create a data set of more natural sentences for training and testing.  
Compound virtual assistant commands are new and not familiar to consumers, this process is error prone also highly dependent on the semantics of the target language.  The success of getting a properly labeled data set depends on the semantics of the formal language. 

{\em Multi-Domain Compositional Semantic Parser}.  The semantic parser for a language like ThingTalk is challenging because it needs to operate across many domains.  
Results for just 2 domains have been reported, with xxx results.
Thingpedia today has over 250 APIs.  This is expected to grow.  We want to support the long tail of programming, and not just the most popular programs.  The challenge is how to support extensibility and accurate parsing of new functions, where there is no adequate data? 

%Related work?  State-of-the-art machine learning algorithms have been proven effective at translating natural to formal languages~\cite{dong2016language, yin2017syntactic, alvarez2016tree, xiao2016sequence, zhong2017seq2sql}, but they usually require large corpora of sentences, annotated with their formal representation.  \TODO{Name the formal languages - this is too broad, the problem for us is multi-domain, and not just that we don't have enough input}. 

%it has a cleaner semantics, matching consumers' conceptual model better, its syntax is also tuned for machine-learning models. 
%providing a superset of functions supported by ThingTalk, it is a semantically cleaner and more compositional language.  This makes it easier for users to understand and use; this also means it is easier to get high-quality training data.  This also makes possible to train a smaller neural model to deliver accurate results.  Syntactically, it is designed to match consumers' conceptual model; for example, it introduces no variables or loops in the language.  Additional considerations are made in designing the syntax to enable  effective semantic parser.

After extensive experimentation with the language and the semantic parser, we have refined ThingTalk to create a language we call \TT, developed a methodology to create a high-quality dataset of manually paraphrased sentences, and created a deep-learning neural model that delivers an accuracy of 88\% on the dataset.  Not only are the semantics and syntax of \TT tuned for translation from natural language, but it is also more expressive than ThingTalk, capable of a superset of functions supported by ThingTalk. 
The knowledge of how natural language can be translated into formal language is given in two parts: NL2FL snippets map NL snippets to API calls, and NL2FL constructs map NL constructs to the constructs in the formal language. The former is embedded in the skill library, the latter is supplied with the \NLPL grammar. 


\fi


==> limitations.tex <==
\section{Limitations \& Future Work}


==> methodology.tex <==
\section{The Genie Methodology}

The output of Genie is a neural network, which synthesizes the formal language from the natural language specification.
In this section, we describe how we acquire data to train the network, and how we can map the synthesis
problem to the neural network sequence-to-sequence model.


==> overview-old.tex <==
\section{Overview}

In this section, we provide an overview of Genie, and how it can be used
to build virtual assistants that support complex tasks and can be extended to new tasks quickly.

\begin{figure*}[tb]
%\includegraphics[figure/user-overview.pdf}
\TODO{figure}
\caption{How a user interacts with a virtual assistant that uses Genie}
\label{fig:user-overview}
\end{figure*}

\subsection{A Virtual Assistant with a Formal Language}

Virtual assistants that use Genie translate every user command into a program, or program fragment, in a well defined programming
language. The user interaction model is shown in Figure~\ref{fig:user-overview}. First, the user's command is
translated from natural language into the agent's programming language; the program is analyzed, and the necessary
libraries and metadata are loaded; then, the program is completed following a fixed slot-filling routine; the agent translates
the program back into natural language and shows it to the user to confirm; finally, the program is executed, the output
is shown to the user and the agent advances to the next state.

\subsection{Defining New Skills with Genie}

Figure~\ref{fig:developer-flow} shows the high-level flow of defining a new task, using Genie.
\begin{enumerate}
\item The developer provides the signature and the implementation of the new primitive in the library.
\item Each signature is annotated with natural language metadata to automatically generate the conversation.
\item The developer provides a list of \textit{code snippets} (parametrized partial programs) with their associated natural language representation.
\item The snippets are combined, using the formal grammar of the programming language, and a simplified
natural language grammar, to produce a large dataset of pairs of synthetic natural language commands and programs.
\item The commands are paraphrased, using crowdsourcing, to produce a training set of real natural language commands and
the associated programs.
\item A combination of paraphrased and synthetic commands is used to train the semantic parser.
\item The trained model is loaded in the virtual assistant, which now understands the newly defined tasks, and can
execute it by loading the implementation on-demand from the library.
\end{enumerate}


==> problem.tex <==
%!TEX root = ./paper.tex
\section{Problem Statement}

\subsection{Advantages of NLPL Languages}

There are many advantages to using an \NLPL language as a formal representation in virtual assistants, provided accurate semantic parsing is achievable.  

\begin{enumerate}
\item Because users can adapt their language based on the capabilities of the assistant, the problem is much easier than general natural language understanding.  For example, we have adapted to Alexa's limitations and learned to write in Graffiti before handwriting recognition became feasible.  

\item \NLPL languages are independent of the choice of natural languages, allowing different semantic parsers to be built, if necessary, for different languages.  For example, strategies for rare languages may be different for common languages. 

\item \NLPL exposes the full capability of the virtual assistant to the deep-learning neural network, instead of introducing an intermediate representation that needs to be interfaced with by both the parser and the execution engine. 

\item 
Commands now have a formal semantics based on \NLPL. This is important because natural language has ambiguity. 

\item
Sophisticated users can write and edit \NLPL programs.  Not only does it let users do what they want, but the inputs can serve as training samples to grow the capability of virtual assistants. 

\item
Tools can be generated based on the formal language.  Genie is one such example as it makes it easy for developers to create parsers for new virtual assistant capabilities.  Brassau is another example that automatically generates a GUI from ThingTalk. 
\end{enumerate}

Machine learning is the well-established technique for natural language processing; however, it requires a large labeled data set, which is not available for new languages. 
Previous attempts in generating compound virtual assistant commands have not been successful.
Semantic parsing on compound virtual assistant commands has been attempted using IFTTT recipe descriptions.  Due to the low quality of inputs (noisy, unintelligible, incorrect), the best accuracy reported was 3\%~\cite{quirk15}.
Hence, to succeed, we need to be able to collect large amounts of high-quality annotated sentence and program pairs. How to do that depends on the design of the formal language, and the methodology used to collect the data.

\subsection{Canonical Program Representation}

Semantic parsing has been used mainly for answering questions. 
Such models can be tested by executing the target program
under a test environment and comparing the output to check whether two programs are equivalent.
This is unsuitable to any domain where programs have side effects, such as IoT commands, and
in practice only applicable to database queries. It is also problematic to apply a neural network
model to such a target language, because standard sequence models that use a syntatic similarity
loss (based on exact match or BLEU scores) are not applicable, and one needs the complex and slow
\textit{dynamic programming on denotations} algorithm introduced by Krishnamurthy et al.~\cite{krishnamurthy2017neural}.

%We also depart from Lambda DCS~\cite{dblp:journals/corr/liang13}, the formal language used by Wang et al.~\cite{overnight}, who introduce the idea of paraphrasing data. 

Many natural language commands can be paraphrased into syntactically different sentences with the
same meaning. We need to tell if the output of our semantic parser is correct.  
It is desirable that whenever two programs are equivalent, there exist a computable
canonical form that is equivalent to both. The machine learning model can then be trained
to produce the canonical form of the program for all paraphrases of any of the program's commands,
regardless how the syntactic structure of the commands.

This means that none of the Turing-complete programming languages has a canonical normal form.
Previous efforts to generate Python have focused exclusively on pseudo-code
readouts of code snippets~\cite{yin2017syntactic}, or have obtained no exact accuracy and resorted
on evaluating on BLEU score, which has no significance for a programming language~\cite{rabinovich2017abstract}.
The full SQL does not have a canonical form either~\cite{trakhtenbrot1950impossibility, chu2017cosette}. Nevertheless, the problem
is tractable for many useful subsets of SQL, and therefore there are many useful sets of commands
that can be mapped to a normalizable formal language~\cite{zhong2017seq2sql}.


%We wish to be able to learn all these paraphrases without annotating each paraphrase separately, as that lets us grow the space of supported commands with significantly less effort.

\subsection{Designing the NLPL to improve accuracy}
The design of the target language affects both the ability to collect data, and the ability of the semantic parser to generalize from limited data.

\iffalse
While model size is not the only factor in the neural network ability to train quickly and generalize
well from small training sizes, it is the one factor that has the most intuitive behavior, and the easiest
to control~\cite{DBLP:journals/corr/ZhangBHRV16,NIPS2017_7176}. In turn, the model size depends
directly on complexity of the target language, in terms of the total number of decoding choices that the
neural network can make, the number of choices that are legal at any given point in the decoding, and the
number of choices needed to decode a specific program.  The smaller the model, the less training data is needed; this is especially important for a new programming language since high-quality training data is hard to acquire.
\fi

\paragraph{Matching the user's mental model}
The closer the formal language is to natural language, the easier
it is to translate. Natural language commands are high-level, succinct and implicit, so
it is desirable for the formal language to do so as well.

\paragraph{Partial Specification Support} %subclasses, parameters

API calls are specific; they often provide many options, and their designs often reflect the underlying implementation.  The users, however, are unaware of all these options. The language needs to accept sentences conveying high-level intent, and infer the details based on either common usage or the context such as the devices the user has.  

For example, it is desirable that the NLPL supports subtyping, to distinguish between general devices and specific brands. This way, when the brand name is omitted the general API can be used.  For example, this lets the system understand a generic phrase like ``send an email'', which can then either prompt the user for specific service or infer it from the resources the user has configured.

\iffalse
The original ThingTalk uses positional parameter passing and unification to connect input and output parameters. That is, an output is passed to any inputs using the same symbol. 
Unification is problematic because variables are given arbitrary names. 
\TODO{Don't understand: that the synthesizer would have to guess, or the user specify the names explicitly in
the sentence.} 
\fi

\iffalse
If the programming language uses positional parameters, then the neural network has to predict
``undefined'' or placeholder values in place of omitted or unspecified parameters; in turn,
this requires the network to learn the exact signature of each function, both order and length.
The signature information is not generalizable across functions, hence the neural network would need massive
amounts of data \textit{for each function} to learn it. Conversely, 
\fi

\iffalse
\paragraph{Precision Tradeoff}
\TODO{Will probably drop unless there is a better argument.}
We found that it is sometimes necessary to trade off precision to improve our ability to get a high-quality training set. 
A concrete example of this
phenomenon is the use of ``greater'' vs. ``greater or equal'' operator: the semantics are similar,
and untrained users are unlikely to think of the edge case in which they differ. Hence, a language
designer should choose one semantic (the one most suitable to the domain) and stick with it.

\iffalse
First of all, the precision of the language has to be limited, so that different
programs can be distinguished by untrained users. If the semantics of two programs are so close
that the users are likely to confuse one for the other, it will not be possible to acquire
a good quality dataset without expensive annotation by experts. 
\fi
\fi

\subsection{Collecting high quality data}

The effectiveness of machine-learning models depends greatly on acquiring a high-quality dataset.
To create a semantic parser for question answering over simple domains, Wang et al. use a syntax-driven approach to create a canonical sentence for each formal program, ask crowdsourced workers to paraphrase canonical sentences to make them more natural, use the paraphrased sentences to train a machine model that can match input sentences against possible canonical sentences~\cite{overnight}.
This approach is inadequate for compositional virtual assistants. 

\paragraph{Coverage}
The training set for the semantic parser must cover all the functions, operators, enumerated values, etc. in the target
formal language.

For virtual assistant in particular, the space of virtual assistant commands is so large that synthetic data generation is the
only option. At the same time, even experts cannot write all possible forms of commands as synthetic sentence
constructs, and not all constructs generalize across the signature library; hence, paraphrasing of individual
sentence sentences is still necessary to achieve generalization.

\paragraph{Challenges of paraphrasing}
%First, we discover empirically that when we show canonical sentences of virtual assistant commands to crowdsourced workers, they often misunderstand the sentences, produce incorrect paraphrases, or change just a few words in the original sentences.  

Virtual assistant commands are much harder than answering questions in a database.
They refer to many domains, each of which has their own natural vocabulary. 
The constructs are also much more powerful and complex.
Without background knowledge, crowdsource workers can be easily confused by
poorly generated synthetic sentences, and when that occurs, they will either paraphrase to a sentence with
a different semantic, or make minimal changes to the input (such as replacing a word they understand with
a synonym), which are not sufficient for training the model.

\subsection{Compositionality} 
The space of virtual assistant commands grows exponentially with the number of functions supported. 
It's impossible to collect a dataset containing all the possible combinations and train a parser on it.
Thus the neural network model needs to generalize to compose unseen programs.

The dataset has to be crafted to teach the model compositionality, and not just a memorization of possible programs.
We have found that a synthetic set is still necessary. Constructs and word choices for the paraphrase prompt must
be limited for understandability, while the training algorithm needs as much variety as possible. Synthetic data
allows to generalize to rare constructs %(e.g., backward parameter passing for ``do when'' or ``use X to do Y'')
that would occasionally appear in inputs but would be hard to understand for a paraphraser.


==> representation.tex <==
\section{Formal Representations in Virtual Assistants}

The design space of a formal representation in a virtual assistant is large.  
The Alexa Abstract Meaning Representation~\cite{banarescu2013abstract}
and the Alexa Meaning Representation Language~\cite{kollar2018alexa, perera2018multi} model natural language phenomena explicitly. They use machine learning to match NL to a representation model which closely matches the semantics of the sentences.  The broadness of the natural language means that this representation model is open-ended.  It is then up to an undefined system to interpret how to perform the action specified.   
These languages have different representations for semantically equivalent sentences.  \TODO{Explain:} This requires complex and expensive manual annotation
by experts, and have to be carefully tuned to match the specifics of the natural language.

At the other end of the spectrum, we can design a formal language that defines precisely what the virtual assistant can execute, leaving it up to the neural network to take full advantage of its capability. ThingTalk is such an example; its design is informed by the capability of the virtual assistant, and not by its amenability to natural language translation.  The reported accuracy so far on a paraphrased dataset is far from practical.  

We advocate the same execution-based approach used in ThingTalk, but the language must be designed to allow for effective natural language translation. Having a formal \NLPL language based on the capability of the virtual assistant has many advantages. 
\begin{enumerate}
\item This representation is independent on the choice of natural languages, allowing different semantic parsers to be used if necessary for different languages.  

\item 
Commands now have a formal semantics based on \NLPL. This is important because natural language has ambiguity. 

\item
Sophisticated users can write and edit \NLPL programs.  Not only does it let users do what they want, but the inputs can serve as training samples to grow the capability of virtual assistants. 

\item
Tools can be generated based on the formal language.  Genie is one such example as it makes it easy for developrs to create parsers for new virtual assistant capabilities.  Brassau is another example that autmatically generates a GUI from ThingTalk. 
\end{enumerate}

It is only through years of experimentation, both in changing ThingTalk, Thingpedia, and the neural network, did we learn how to design such \NLPL languages.  


==> results.tex <==
%!TEX root = ./paper.tex
\section{Design Rationale}
When designing a \NLPL language, the first priority is to ensure that it has a (unique) canonical representation because machine learning depends on it, and the next is the ability to create an effective parser. 

\subsection{Canonical Program Representation}

Semantic parsing has been used mainly for answering questions. 
Such models can be tested by executing the target program
under a test environment and comparing the output to check whether two programs are equivalent.
This is unsuitable to any domain where programs have side effects, such as IoT commands, and
in practice only applicable to database queries. It is also problematic to apply a neural network
model to such a target language, because standard sequence models that use a syntatic similarity
loss (based on exact match or BLEU scores) are not applicable, and one needs the complex and slow
\textit{dynamic programming on denotations} algorithm introduced by Krishnamurthy et al.~\cite{krishnamurthy2017neural}.

%We also depart from Lambda DCS~\cite{dblp:journals/corr/liang13}, the formal language used by Wang et al.~\cite{overnight}, who introduce the idea of paraphrasing data. 

Many natural language commands can be paraphrased into syntactically different sentences with the
same meaning. We need to tell if the output of our semantic parser is correct.  
It is desirable that whenever two programs are equivalent, there exist a computable
canonical form that is equivalent to both. The machine learning model can then be trained
to produce the canonical form of the program for all paraphrases of any of the program's commands,
regardless how the syntactic structure of the commands.

This means that none of the Turing-complete programming languages has a canonical normal form. The full SQL does not either~\cite{trakhtenbrot1950impossibility, chu2017cosette}. Nevertheless, the problem
is tractable for many useful subsets of SQL, and therefore there are many useful sets of commands
that can be mapped to a normalizable formal language.

\TODO{Describe how we make it canonical}

%We wish to be able to learn all these paraphrases without annotating each paraphrase separately, as that lets us grow the space of supported commands with significantly less effort.

\subsection{Effectiveness of Semantic Parsing}
While model size is not the only factor in the neural network ability to train quickly and generalize
well from small training sizes, it is the one factor that has the most intuitive behavior, and the easiest
to control~\cite{DBLP:journals/corr/ZhangBHRV16,NIPS2017_7176}. In turn, the model size depends
directly on complexity of the target language, in terms of the total number of decoding choices that the
neural network can make, the number of choices that are legal at any given point in the decoding, and the
number of choices needed to decode a specific program.  The smaller the model, the less training data is needed; this is especially important for a new programming language since high-quality training data is hard to acquire.

\paragraph{Matching the user's mental model}
The closer the formal language is to natural language, the easier
it is to translate. Natural language commands are high-level, succinct and implicit, so
it is desirable for the formal language to do so as well.

The original ThingTalk design reflects this principle well.
It is more natural for users to think about subsets of data with certain characteristics, rather than the execution paths. Thus it is data focused and not control flow focused. Instead of explicit looping constructs, ThingTalk uses implicit looping and implicit
scalarization of list data structures. Similarly, it uses filters rather than if statements.

%Explicit variables should also be avoided, as the user will not use explicit names for the
intermediate results in their commands.

\paragraph{Semantically Orthogonal Components}
ThingTalk was designed to extend trigger-action computation model, made popular by IFTTT, with the ability to compose functions.  Thus, it has three clauses: {\em when} an event happens, {\em get} some data, and {\em do} some operation.  They map directly to three kinds of function implementations in Thingpedia: {\em callbacks}, {\em retrievals}, and {\em actions}. Unfortunately, the semantics of callbacks and queries are not easily discernible to consumers.  It is hard for users to understand that ``when Trump tweets'' and ``get a Trump tweet'' refer to two different functions. Furthermore, when a device supports only a callback and not a retrieval, or vice versa, the user will not be able to learn when they are allowed to call which.  

In \TT, we collapse the distinction between callbacks and queries into one class: queries, which can be monitored as event or used to get data.  The \TT runtime ensures that any supported retrieval can be monitored as events, and vice versa. Not only does this give the system more functionality, we make the language more orthogonal, which is useful to both the user and the parser.

%Empirically, we observe that even after this change, about 3\% of our test data is ambiguous with respect of \texttt{now} vs. \texttt{monitor}, so reducing the effect of ambiguity is critical.

\paragraph{Partial Specification Support} %subclasses, parameters

API calls are specific; they often provide many options, and their designs often reflect the underlying implementation.  The users, however, are unaware of all these options. The language needs to accept sentences conveying high-level intent, and infer the details based on either common usage or the context such as the devices the user has.  

\TT supports subtyping to distinguish between general devices and specific brands, so that when the brand name is omitted the general API can be used.  For example, this lets the system understand a generic phrase like ``send an email'', which can then either prompt the user for specific service or inferred from the resources the user have configured.

\TT uses keyword parameters, rather than the more conventional positional parameters. 
When using keyword
parameters the neural network only needs to learn the partial signature of the functions, and not 
the length of the signature.  
The order of parameters in the prediction is defined globally by the canonical form; hence, the language model of parameters can generalize across functions.  This greatly reduces the model size and the training data size requirement. 

The original ThingTalk uses positional parameter passing and unification to connect input and output parameters. That is, an output is passed to any inputs using the same symbol. 
Unification is problematic because variables are given arbitrary names. 
\TODO{Don't understand: that the synthesizer would have to guess, or the user specify the names explicitly in
the sentence.} 

\TT simply uses declared parameter names to indicate parameter passing. 
\TODO{Describe the cat example.}
No new variables are introduced, and the model only needs to learn the parameter names associated with each function. In other words, 
To increase compositionality, we encourage developers to use the same naming conventions so the same parameter names are used for similar purposes. 
\TODO{Give example}. 
In the case, where two functions in the same command use the same parameter names, we resolve the conflict by assuming that the name refers to the rightmost instance. Here we consciously trade off completeness for accuracy in the common case. 

Besides changing the original ThingTalk syntax, we also need to change the content in Thingpedia to support partial specification.  Where possible, we should collapse multiple functions into one, and use parameters to distinguish between them.  For example, gmail has three functions ``receive\_email'', ``receive\_important\_email'', ``receive\_primary\_email'' for reading mails in the inbox, starred messages, and primary messages (not promotion, social, etc), respectively. We combine them into ``receive\_email'' and add an optional parameter to indicate the category of mail.  If the user does not specify the kind of mail, the inbox is assumed.  Parameterization has two advantages: 
(1) the neural network is not forced to make an immediate
hard decision, and can defer the decision after choosing the function (and receiving positive
reward for it), (2) if the sentence is ambiguous, the neural network can a produce a
partially correct answer 100\% of the time. 
This improves training and reduces the negative effect of ambiguous sentences in
the training set.

\iffalse
If the programming language uses positional parameters, then the neural network has to predict
``undefined'' or placeholder values in place of omitted or unspecified parameters; in turn,
this requires the network to learn the exact signature of each function, both order and length.
The signature information is not generalizable across functions, hence the neural network would need massive
amounts of data \textit{for each function} to learn it. Conversely, 
\fi

\paragraph{Compositionality} % Adding types to the programs
\TODO{Add this point}
The space of virtual assistant commands grows exponentially with the number of functions supported. 
It's impossible to collect a dataset containing all the possible combinations and train a parser on it.
Thus the neural network model needs to generalize to compose unseen programs. 


\paragraph{Precision Tradeoff}
\TODO{Will probably drop unless there is a better argument.}
We found that it is sometimes necessary to trade off precision to improve our ability to get a high-quality training set. 
A concrete example of this
phenomenon is the use of ``greater'' vs. ``greater or equal'' operator: the semantics are similar,
and untrained users are unlikely to think of the edge case in which they differ. Hence, a language
designer should choose one semantic (the one most suitable to the domain) and stick with it.

\iffalse
First of all, the precision of the language has to be limited, so that different
programs can be distinguished by untrained users. If the semantics of two programs are so close
that the users are likely to confuse one for the other, it will not be possible to acquire
a good quality dataset without expensive annotation by experts. 
\fi

%No intermediate language because of neural network. 
%LambdaDCS works on a subset of SQL - 

\paragraph{Lessons Learned for Data Collection}

Our results show the importance of obtaining a comprehensive, high quality dataset for semantic parsing: 
while machine learning improvements can help, they are secondary if the data is just not there for the task at hand.

In particular, the training set must cover all the operators, enumerated values, measurement units, etc. in the target
formal language. For virtual assistant in particular, the space is so large that synthetic data generation is the
only option. At the same time, even experts cannot write all possible forms of commands as synthetic sentence
constructs, and not all constructs generalize across the signature library; hence, paraphrasing of individual
sentence sentences is still necessary to achieve generalization.

Yet, paraphrasing of virtual assistants commands, which span many domains and are unfamiliar to
users, is not an easy task. Without background knowledge, crowdsource workers can be easily confused by
poorly generated synthetic sentences, and when that occurs, they will either paraphrase to a sentence with
a different semantic, or make minimal changes to the input (such as replacing a word they understand with
a synonym), which are not sufficient for training the model.

At the beginning, in designing the constructs, we matched the formal language closely. This did not generalize well,
so we restarted from natural language (what and how users might want to say), and wrote the corresponding formal language for each construct.
We leveraged domain knowledge, existing repositories, and previously collected paraphrases to refine the constructs.

We have spent more than 2 years refining data collection for Genie, and in the process we have learned
the following practical considerations that improve the understandability of synthetic sentences:
\begin{itemize}
\item We noticed that ungrammatical sentences in particular correlate with mistakes, so tuned the snippets and templates to make the sentences grammatically correct.
\item We introduced the code snippet to account for less general grammar forms, and over time reduced our reliance on general constructs. % (e.g., ``when I receive an email'' vs ``when my emails changes'')
\item We worked with Thingpedia contributors and revised the library to ensure that the natural language corresponding to all components of the same type have the same grammar category (e.g., all parameter names need to be noun phrases).
\item We found it important to choose grammar categories that compose naturally. Our original design used only verb phrases for queries (commonly of the form ``get X''), but we switched to primarily noun phrases as they support composition by replacement (e.g., ``a cat picture'' can be replaced in ``post X on Twitter'' and ``post X on Facebook'', while ``get a cat picture'' cannot).
\item Functions in the library should be finely categorized to generate more meaningful commands. In \TT, we introduced the distinction of \textit{list} and \textit{monitorable} functions.
\item The complexity of the program (in terms of parameter passing and filters) must be limited, or the sentence becomes unintelligible.

\item As parameters are chosen automatically, it is helpful to workers to annotate them in the prompts (using quotes or @-signs), and to choose the values carefully in a way that is both general and meaningful.

\item As a result of exhaustive enumeration, the synthetic set contains unusual combinations of functions or parameters, that can be confusing to a non expert.
For example, the combination $\text{@com.gmail.inbox} \Rightarrow \text{@com.gmail.send}$ is problematic because it looks like an auto-reply, but reply functionality should use the @com.gmail.reply function to preserve threading correctly. Genie provides an interface to blacklist certain function combinations, and control the sampling of synthetic sentences for paraphrasing.
\item We found it useful in particular to pair less common devices with widely recognized ones in compound commands.
\item We also provided hints in the paraphrasing interface with description of less common brand names.
\end{itemize}

In parallel to the data collection process, we have worked on the semantic parsing, and we have found
that a synthetic set is still necessary. We have found it crucial to subset the constructs and word choices for
the paraphrase prompt, while exposing more variety to the training algorithm. Synthetic data also allowed
us to generalize some rare constructs (e.g., backward parameter passing for ``do when'' or ``use X to do Y'')
that would occasionally appear in inputs but would be hard to understand for a paraphraser.

And of course, all the usual hints related to crowdsourcing apply: workers will try to cheat, they will
try to get away with minimal work, they will not read the instructions. Automatic and manual validation
helps with errors and cheating. To encourage variety and effort, we found that asking two paraphrases for each prompt
was the optimal equilibrium: people will have a hard time writing three different paraphrases, and conversely
with only one they will tend to make the most obvious changes.

\iffalse
We need a lot of data to train the semantic parser
\begin{itemize}
\item We need coverage of all the operators, enums, units, etc -> we need synthetic.
\item We can never write down all the possible templates to generate synthetic sentences. Not all templates generalize to all devices -> we need paraphrase.
\item Use the synthetic dataset for regularization (e.g., ``?'', ``.'')
\item Use ``choice'' to have more variety with a single construct.
\end{itemize}

Turkers can easily be confused by the synthetic sentences, and as a result, 
they either paraphrase the sentence with a different meaning, or only make minimum changes (only change a word). 
\begin{itemize}
\item We need to show understandable synthetic
    
\item Provide hints to explain less common devices.
\item Carefully design the constructs
    \begin{itemize}
    \item Start from natural language (what and how users might want to say).  
    \item Leverage domain knowledge, existing repositories, previous collected paraphrase to refine templates
    \item constructs need iterations
    \item Categorize function to get more meaningful commands (e.g., list, monitorable)
    \item Subset the constructs and choices for turking: use more general/common words and construct
    \item Some rare constructs are still needed for synthetic. (e.g., backward parameter passing for ``do when''; ``use X to do Y'')
    \item Limit the formal language to those can be expressed in natural language. 
    \end{itemize}
\end{itemize}


Even if turkers understand the sentence, they still make mistakes, and some of them try to cheat. 
They also tend to only make small changes.
\begin{itemize}
\item Hire masters
\item Turkers don't read the instructions carefully. 
\item Automatic validation based on heuristic, string match, etc.
\item Manual validation to check the meaning of the paraphrases
\item Automatic validation on the manual validation: validators are also humans and they try to cheat.
\item Ask for 2 paraphrases per turker per synthetic sentence to introduce more variety. (2 is the magic number, 3 will introduce too much garbage)
\item Typos are common in paraphrase but the spell check doesn't work well because of all the brand names, service name, domain-specific words.
\end{itemize}
\fi


==> thingpedia.tex <==
%!TEX root = paper.tex
\section{Representing and Growing The Space of ThingTalk Programs}
ThingTalk has a very simple control construct, but it is powerful as it is designed to work with 
Thingpedia.

\subsection{Thingpedia}
Thingpedia is an encyclopedia of IoT devices and Internet services. 
It is an open-source, non-proprietary, and crowdsourced repository that holds the full
signature of the APIs: it captures not just the input parameters, but also the return results.
It maps high-level natural language commands, onto different implementations for different providers.
Each Thingpedia entry contains a class, a dataset, and some metadata.

\subsection{Classes in \TT}
The methods supported by each Thingpedia entry is defined in a {\em class}, 
where the class name is preceded by the ``@'' sign.
Each class declares the methods the device supports, as well as the module type and configuration 
method. 

\subsubsection{Method Declarations}
Each method declaration has 
a method type (query or action), a name, and a list of parameter declarations.
A query can have two optional modifiers {\em monitorable} and {\em list}.
The former indicates the method can be monitored as a {\em stream};
the latter indicates the method returns a list of results. 
A method named $\mathit{fn}$ in class named $\mathit{cn}$ is referred to as $\mathit{@cn.fn}$.

\subsubsection{Parameter Declarations}
Each parameter has a modifier, name, and type.
The modifier {\em in req} designates a required input parameter,
{\em in opt} designates an optional parameter, 
and {\em out} designates an output parameter.
Action can not have output parameters.

Strong typing is used in \TT to help the translation from natural language.
Moreover, as \TT is used to connect different methods together, 
type checking can help ensure that the parameters from different methods
are connected in the right way.

\TT has standard types including strings, numbers, booleans, and enumerated types.
It also has common object types used in IoT devices and web services,
such as measurements, locations, pictures, currencies.
\TT also has entity types that include:
date, time, usernames, email addresses, phone numbers, hashtags, file names, and URLs.
Developers can also define custom entities for their domain-specific tasks.
Finally, ThingTalk also has arrays as the single compound type supported.

\subsubsection{Class Inheritance}
\TT supports one explicit level of multiple inheritance.
A subclass $c_1$ {\em extends} $c_2$ means that it inherits all the method declarations
in $c_2$. 
For example, a specific brand of thermostat may inherit from a generic thermostat class
and have extra methods only available with that brand. 


\subsection{Synthetic Data Generation}
Every kind of device has its own set of operations and hence vocabulary. 
To support natural language understanding and interaction with users, 
each Thingpedia entry includes 
a dataset contains {\em composable code snippets} and their corresponding natural language utterances.
The dataset is used to generate synthetic sentences based a {\em general natural language grammar}.
Then the generated data will be used for training, as well as paraphrasing to collect 
more natural sentences. 

A {\em composable code snippet} has a type, a name, a list of arguments, 
a \TT function, and a list of corresponding natural language utterances.
Each code snippet could have type stream, query, or action.
The name is optional. 
When the name is given, the code snippet can be reused as part of other code snippets within the same dataset file.
The \TT function describes a stream, a query, or an action, according to the type,
by invoking one or more methods. 
The utterances provide different ways of expressing the function.

Each code snippet can also specify the arguments it uses, which can be referred in the code and utterances. 
For example, the following code snippet provides the code and utterances for the action 
to post something on LinkedIn.

\begin{tabbing}
123\=1234\=5678901234\=\kill
\>$\texttt{action}~~\text{(p\_status: String)}$\\
\>\>:= @com.linkedin.share(status = p\_status)\\
\>\#\_[utterances=["share \$p\_status on linkedin", \\
\>\>\>"post \$p\_status on linkedin"]]\\
\end{tabbing}

It defines the argument {\em p\_status} and uses it as a placeholder in the utterances.
The placeholder then can be replaced with different values to generate sentences.
 
Each code snippet can be used to compose a \TT program. 
The input of each code snippet is the specified arguments and they are considered as required.
The output parameters will be inferred based on the method it uses.

\subsubsection{Parameter Values}
To bootstrap the machine learning with more data, developers can provide example values when
declaring a parameter. 
The values will used to generate more realist synthetic sentences.

\subsection{Representing Outputs}
When a stream or a query is combined with the default action {\em notify}, the returned results will be 
presented to the user in Almond. 
Since methods in Thingpedia can have multiple output parameters in various types, it is important 
to present the results properly.

Developers can specify how they wish the results will be presented with {\em formatted} annotation
for each query method. 
Three types of outputs are supported: (1) text: which simply returns a string;
(2) picture: which shows a picture based on the URL of the image;
(3) RDL: which returns a clickable link with a title and a description. 

Developers can choose what parameters to present in each type, and parameters can be omitted.
Furthermore, if the developers need more control over the output, such as different output based on results,
they can pass in Javascript code to present the results in a customized way.

\subsection{Design Rationale}


==> thingtalk.tex <==
\section{The \TT Programming Language}

\subsection{Program Syntax \& Semantics}
\TT is a domain-specific language that we designed, specifically optimized to build virtual assistants. It has a single
control construct:
\begin{align}
\textit{stream}\Rightarrow\textit{query}\Rightarrow\text{action}\nonumber
\end{align}

The \textit{stream} portion of the program defines when the program should be evaluated, as a continuous stream
of events. The optional \textit{query} defines additional data that should be retrieved when the program is triggered.
The \textit{action} defines what the program should do.

Stream, query and action invoke methods defined in an external library of ThingTalk classes. 
There are two types of methods: \textit{query methods} retrieve data and have no side-effects, while
\textit{action methods} have side-effects but do not return data.

Specifically, the stream can be the degenerate stream \texttt{now}, which triggers the program once immediately, or it can
be a \texttt{monitor} of a query. The query is constructed as the join of one or more invocations of a query method.
as well as predicates constructed by invoking an arbitrary query method and computing on its output.
The action invokes the builtin \texttt{notify}, which presents the result to the user, or one or more action methods defined in the library.

To allow translation to and from natural language, \TT uses named parameters for inputs and outputs.
Action methods have only input parameters, while query methods have both input and output parameters;
output parameters can be named in subsequent method invocations to pass data from one method to the next.
To avoid naming conflicts, queries can be renamed using an \textit{alias}, which introduces a prefixed
namespace for the output parameters. Otherwise, by default parameters of later functions (to the right
of a join or arrow) shadow the earlier ones.
The design avoids as much as possible the introduction of arbitrary names in the program, so that the
user does not need to specify them exactly in their command.

Output parameters can also be used in a boolean predicate applied to the output of each query to filter
its output, using equality, comparison, string and array containment. Additionally, the filter can
itself refer to an invocation of an arbitrary query method, followed by a boolean predicate on the
outputs of that method.

The distinction of query methods and action methods provides freedom to the synthesizer and optimizer routines:
the portion of the program before the action can be rearranged and modified without visible side effects,
provided that the action is still called the current number of times.

\subsection{Design Rationale}

\TT is designed to be elegant for users to express trigger-action commands in natural language. Natural language translation is made possible by the use of very high-level functions, which are annotated with a natural language description, and by the use of named parameters, which can appear in any order, and whose natural language paraphrases can be learned from data.

In \TT, following the experience of IFTTT, all accounts are named implicitly based on a list of accounts and credentials that is maintained for the user. A \TT program need not specify which Twitter account or which GMail account, knowing that the runtime will pick the one that belongs to the user.

\TT supports optional input parameters, and can represent unspecified required input parameters; thus, the same function can be used with commands that have different combinations of parameters. The fewer the functions to choose from, and the more sentences mapping to the same function, the more precisely the synthesizer will learn the semantics of the function.

Virtual assistant programming often involves operating on sets of data, where selected information from one account is used in another.  The user is given the abstraction that they are describing operations on scalars.  \TT handles list data by letting each method return a list of records. This list is implicitly traversed and the output parameters of the function are bound to each element in the list one at a time, in a fashion similar to list monads or list comprehensions.  The parameters can be filtered by a predicate, so actions are applied only to a subset of the list.  By implicitly looping over the results, we avoid having the user specify traditional loop constructs, which also makes synthesis easier.

\subsection{General Natural Language Grammar}
To generate synthetic sentences with more variety, a general natural language grammar has been designed.
A small subset of the grammar is presented as follows:

\begin{flalign*}
&\text{\ACTION}[a] \rightarrow \text{\PROGRAM}[\text{now} \Rightarrow a]\\
&\text{get | show } \text{\QUERY}[q]  \rightarrow \text{\PROGRAM}[\text{now} \Rightarrow q \Rightarrow \text{notify}]\\
&\text{\STREAM}[s] \text{ notify me | let me know }  \rightarrow \text{\PROGRAM}[s \Rightarrow \text{notify}]\\
&\text{\STREAM}[s] \text{ then } \text{\ACTION}[a] \rightarrow \text{\PROGRAM}[s \Rightarrow a]\\
&\text{\ACTION}[a] \text{ \STREAM}[s] \rightarrow \text{\PROGRAM}[s \Rightarrow a]\\
&...
\end{flalign*}

The explanations for each grammar rule are:
\begin{enumerate}
\item The utterance of an action snippet, is the canonical sentence for the program
generated by adding the stream {\em now} to the action.
\item If we add a random generic verb such as ``get'' and ``show'' before the utterance of a query snippet,
we get the sentence for a program created by adding the stream {\em now} and action {\em notify} to the query.
\item If we add ``notify me'' or ``let me know'' after the utterance of a stream snippet, 
then we get the sentence for a program created by adding the action {\em notify} to the stream.
\item If we have a sequence: the utterance of a stream snippet, ``then'', the utterance of an action snippet,
we get the sentence for a stream-action program.
\item we can also get the sentence for the same stream-action program by putting the utterance of the action
in front of the one of the stream.
\end{enumerate} 

The same program can have multiple grammar rules to generate sentences with more variety. 
For example, suppose we have utterance 
``when New York Times article changes'' for \texttt{monitor (@com.nytimes.get\_front\_page())}
and ``send an email'' for \texttt{@com.gmail.send\_email()}.
Based the fourth and fifth grammar rules we can generate 
``when New York Times article changes, then send an email'' and ``send an email when New YorkTimes article changes'' for the program
\texttt{monitor (@com.nytimes.get\_front\_page()) $\Rightarrow$ @com.gmail.send\_email(). }


==> tt-design.tex <==
\section{Design Principles for Programmable Virtual Assistants}

Our goal is to support building accurate and expressive virtual assistants with small
effort. Part of that goal depends on designing the target language in a way that makes it possible.
In this section, we present some of the challenges and design principles that guide this design.

\paragraph{Matching the user's mental model}
The closer the formal language is to the correspondent natural language, the easier
it is to translate. Natural language commands are high-level, succinct and implicit, so
it is desirable for the formal language to do so as well.

One practical consideration to match the user's mental model is to describe the
execution in terms of data, through predicates and quantifiers, rather than control flow.
We recommend to avoid explicit looping constructs, in favor of implicit looping and implicit
scalarization of list data structures. Similarly, it is better to use filters than if statements,
as it is more natural for users to think about subsets of data with certain characteristics, rather than which path
should the program follow.

Explicit variables should also be avoided, as the user will not use explicit names for the
intermediate results in their commands.

\paragraph{Ambiguity}
Natural language is inherently ambiguous, and the design of the formal language must account
for that.

First of all, the precision of the language has to be limited, so that different
programs can be distinguished by untrained users. If the semantics of two programs are so close
that the users are likely to confuse one for the other, it will not be possible to acquire
a good quality dataset without expensive annotation by experts. A concrete example of this
phenomenon is the use of ``greater'' vs. ``greater or equal'' operator: the semantics are similar,
and untrained users are unlikely to think of the edge case in which they differ. Hence, a language
designer should choose one semantic (the one most suitable to the domain) and stick with it.

Secondly, the formal language should be designed to express ambiguous programs with an exact
representation. This way, the neural network need not choose arbitrarily one of the possible
interpretations. For example, it is better to use parameters to distinguish similar semantics,
rather than different functions, because parameters can be omitted when the sentence is ambiguous,
resulting in an exact representation of the sentence, even if incomplete. The language
should also use subtyping to distinguish between general devices and specific brands, so that when
the brand name is omitted the general API can be used.

\paragraph{Program normalization}
Many natural language commands can be paraphrased into syntactically different sentences with the
same meaning. We wish to be able to learn all these paraphrases without annotating each paraphrase
separately, as that lets us grow the space of supported commands with significantly less effort.
To do so, it is desirable that whenever two programs are equivalent, there exist a computable
canonical normal form that is equivalent to both. The machine learning model can then be trained
to produce the normal form of the program for all paraphrases of any of the program's commands,
regardless how the syntactic structure of the commands.

Note that this rules out languages such as full SQL, for which program equivalence is undecidable
in the general case~\cite{trakhtenbrot1950impossibility, chu2017cosette}. Nevertheless, the problem
is tractable for many useful subsets of SQL, and therefore there are many useful sets of commands
that can be mapped to a normalizable formal language.

This design principle is also a departure from existing languages such as Abstract Meaning Representation~\cite{banarescu2013abstract}
and the Alexa Meaning Representation Language~\cite{kollar2018alexa, perera2018multi}, which
instead model natural language phenomena explicitly. These languages have different representations
for semantically equivalent sentences, and therefore require complex and expensive manual annotation
by experts, and have to be carefully tuned to match the specifics of the natural language.

We also depart from Lambda DCS~\cite{dblp:journals/corr/liang13}, the formal language used by Wang et al.~\cite{overnight},
who introduce the idea of paraphrasing data. Their model relies on executing the target program
under a test environment and comparing the output to check whether two programs are equivalent.
This is unsuitable to any domain where programs have side effects, such as IoT commands, and
in practice only applicable to database queries. It is also problematic to apply a neural network
model to such a target language, because standard sequence models that use a syntatic similarity
loss (based on exact match or BLEU scores) are not applicable, and one needs the complex and slow
\textit{dynamic programming on denotations} algorithm introduced by Krishnamurthy et al.~\cite{krishnamurthy2017neural}.

\paragraph{Size of the neural network models}
While model size is not the only factor in the neural network ability to train quickly and generalize
well from small training sizes, it is the one factor that has the most intuitive behavior, and the easiest
to control~\cite{DBLP:journals/corr/ZhangBHRV16,NIPS2017_7176}. In turn, the model size depends
directly on complexity of the target language, in terms of the total number of decoding choices that the
neural network can make, the number of choices that are legal at any given point in the decoding, and the
number of choices needed to decode a specific program.

In Genie, the neural network model uses a representation based on bottom-up grammar productions. This
means that the designer of the formal language should design the grammar to reduce the overall number of
rules, while at the same time minimizing the number of productions needed for a program. Furthermore,
to reduce the number of grammar productions that are legal at any point, the grammar should encode at least
part of the type system. For example, rather than a single grammar rule of the form:
$$\textit{parameter} \rightarrow \textit{identifier} \texttt{ = } \textit{constant}$$
it is preferrable to use a rule of the form:
$$\textit{parameter\_String} \rightarrow \textit{identifier\_param\_String} \texttt{ = } \textit{string\_literal}$$
and similarly for other types. Using such an encoding, the conditional probabilities of consecutive grammar rules
become independent on the input sentence, which makes them easier to learn.

\subsection{Optimizing the Template Grammar}

